Solving Interpretable Kernel Dimension Reduction

Kernel dimensionality reduction (KDR) algorithms find a low dimensional representation of the original data by optimizing kernel dependency measures that are capable of capturing nonlinear relationships. The standard strategy is to first map the data into a high dimensional feature space using kernels prior to a projection onto a low dimensional space. While KDR methods can be easily solved by keeping the most dominant eigenvectors of the kernel matrix, its features are no longer easy to interpret. Alternatively, Interpretable KDR (IKDR) is different in that it projects onto a subspace \textit{before} the kernel feature mapping, therefore, the projection matrix can indicate how the original features linearly combine to form the new features. Unfortunately, the IKDR objective requires a non-convex manifold optimization that is difficult to solve and can no longer be solved by eigendecomposition. Recently, an efficient iterative spectral (eigendecomposition) method (ISM) has been proposed for this objective in the context of alternative clustering. However, ISM only provides theoretical guarantees for the Gaussian kernel. This greatly constrains ISM's usage since any kernel method using ISM is now limited to a single kernel. This work extends the theoretical guarantees of ISM to an entire family of kernels, thereby empowering ISM to solve any kernel method of the same objective. In identifying this family, we prove that each kernel within the family has a surrogate $\Phi$ matrix and the optimal projection is formed by its most dominant eigenvectors. With this extension, we establish how a wide range of IKDR applications across different learning paradigms can be solved by ISM. To support reproducible results, the source code is made publicly available on \url{https://github.com/chieh-neu/ISM_supervised_DR}.

==> tex/e_on_HSIC.tex <==
\section{An Overview on HSIC}
Proposed by \citet{gretton2005measuring}, the Hilbert Schmidt Independence Criterion (HSIC) is a statistical dependence measure between two random variables. HSIC is similar to mutual information (MI) because given two random variables $X$ and $Y$, they both measure the distance between the joint distribution $P_{X,Y}$ and the product of their individual distributions $P_X P_Y$. While MI uses KL-divergence to measure this distance, HSIC uses Maximum Mean Discrepancy~\cite{gretton2012kernel}. Therefore, when HSIC is zero, or $P_{X,Y}=P_X P_Y$, it implies independence between $X$ and $Y$. Similar to MI, HSIC score increases as $P_{X,Y}$ and $P_X P_Y$ move away from each other, thereby also increasing their dependence. Although HSIC is similar to MI in its ability to measure dependence,  it is easier to compute as it removes the need to estimate the joint distribution. 

%Due to this advantage, HSIC has been applied to a wide range of applications, e.g., independence hypothesis testing \citep{gretton2008kernel}, dimensionality reduction \cite{niu2011dimensionality, suzuki2010sufficient}, feature selection \cite{song2007supervised}, and alternative clustering \cite{niu2014iterative,wu2018iterative}.








Formally, given a set of $N$ i.i.d. samples $\{(x_1,y_1),...,(x_N,y_N)\}$ drawn from a joint distribution $P_{X,Y}$. Let $X \in \mathbb{R}^{N \times d}$ and $Y  \in \mathbb{R}^{N \times c}$ be the corresponding sample matrices where $d$ and $c$ denote the dimensions of the datasets. We denote by $K_X,K_Y \in \mathbb{R}^{N \times N}$ the kernel matrices with entries $K_{X_{i,j}}=k_X(x_i,x_j)$ and $K_{Y_{i,j}} = k_Y(y_i,y_j)$, where $k_X: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$ and $k_Y: \mathbb{R}^c \times \mathbb{R}^c \rightarrow \mathbb{R}$ represent kernel functions. Furthermore, let $H$ be a centering matrix defined as $H=I_n - \frac{1}{n} \textbf{1}_n\textbf{1}_n^T$ where $\textbf{1}_n$ is a column vector of ones. HSIC is computed empirically with
%Formally, given two datasets $X \in \mathbb{R}^{n \times d}$ and $Y  \in \mathbb{R}^{n \times c}$, where $n$ denotes the number of samples while $d$ and $c$ denote the dimensions of the datasets. We further denote the kernels computed from each dataset as $K_X \in \mathbb{R}^{n \times n}$ and $K_Y \in \mathbb{R}^{n \times n}$. HSIC can be computed empirically with
\begin{equation}
    \mathbb{H}(X,Y) = \frac{1}{(n-1)^2} \Tr(K_X H K_Y H).
    \label{eq:emprical_hsic}
\end{equation}
%Here, $K_X$ is assumed to be Gaussian and $K_Y$ is assumed to use a linear kernel. $H$ in this context is a centering matrix that is symmetric and defined as 
%$H=I_n - \frac{1}{n} \textbf{1}_n\textbf{1}_n^T$ where $\textbf{1}_n$ is a column vector of length $n$ with element of all 1s. 




%To clarify HSIC's relationship to MI, we note that MI$(X,Y)$ compute the dependency between $X$ and $Y$ by finding the KL-divergence between the joint distribution $P_{X,Y}$ and the product of their individual distributions $P_XP_Y$. Similarly, HSIC compares $P_{X,Y}$ and $P_XP_Y$ via another measure called Maximum Mean Discrepancy (MMD). Therefore, 
%when the MMD distance between $P_{XY}$ and $P_XP_Y$ is 0, or $P_{XY} = P_XP_Y$, it implies a complete independence between $X$ and $Y$. Conversely, a high $\mathbb{H}(X,Y)$ implies a high dependency between $X$ and $Y$. Based on its ability to measure dependence, it allows HSIC to become a powerful tool for dimension reduction. A common strategy is to discover a projection matrix $W$ to project the data $X$ into a lower dimension while maintaining a high HSIC against some known lables $Y$. 



%MMD measures the difference between distributions by matching the moments of the distributions with characteristic kernels. Therefore, $MMD(P_{X,Y},P_XP_Y)=0$ if and only if $P_{X,Y} = P_XP_Y$ \cite{sejdinovic2013equivalence,li2017mmd}. Given this relationship, $\mathbb{H}(XW,Y) = 0$ implies an independence between $XW$ and $Y$. Conversely, if $\mathbb{H}(XW,Y)$ is maximized, $XW$ and $Y$ becomes highly dependent. 




















%Originally proposed by \cite{gretton2005measuring}, HSIC is a statistical dependence measure between two distributions.
%Whereas Pearson correlation coefficient \cite{benesty2009pearson} only measures the linear dependence between variables, HSIC also captures non-linear relationships. 
%Although mutual information can also detect non-linear relationships, the empirical HSIC is significantly easier to compute. Here we provide the definition and interpretation of HSIC.  
%
%Given $x \sim \mathcal{X}$ and $y \sim \mathcal{Y}$, we define two feature maps $\phi$ and $\psi$ that correspondingly maps $x$ and $y$ into the Reproducing Kernel Hilbert Spaces (RKHS) of $\mathcal{F}$ and $\mathcal{G}$. We next define $\mu_x=E[\phi(x)]$ and $\mu_y=E[\psi(y)]$. The definition of HSIC is centered around the cross covariance operator $C_{X,Y}$ that is defined as 
%\begin{equation}
%    C_{X,Y} = \E_{X,Y}[(\phi(x) - \mu_x)(\psi(y) - \mu_y)^T]. 
%    \label{eq:cross_cov}
%\end{equation}
%It can be seen that the definition of cross covariance operator is reminiscent of the covariance matrix, except that the data is first projected onto the RKHS. With this insight HSIC is defined as the Hilbert-Schmidt norm of the $C_{X,Y}$
%\begin{equation}
%    \HSIC(X,Y) = ||C_{X,Y}||_{HS}^2
%\end{equation}
%Since infinite samples are required to compute Eq. (\ref{eq:cross_cov}), HSIC is often computed empirically with  
%\begin{equation}
%    \HSIC(X,Y) = \frac{1}{(n-1)^2} \Tr(K_X H K_Y H),
%    \label{eq:emprical_hsic}
%\end{equation}
%where $n$ is the number of sample, $K_X$ and $K_Y$ are kernel matrices computed from variables $X$ and $Y$. $H$ in this context is a centering matrix defined as 
%$H=I_n - \frac{1}{n} \textbf{1}_n\textbf{1}_n^T$ where $\textbf{1}_n$ is defined as a column vector of length $n$ and all element of 1s.
%
%HSIC's ability to measure dependence between two variables also has interpretations in information theory. While mutual information of $X$ and $Y$ is the KL-divergence between $P_{X,Y}$  and $P_XP_Y$, $\HSIC(X,Y)$ is the Maximum Mean Discrepancy (MMD) 
%between $P_{X,Y}$ and $P_XP_Y$ \cite{sejdinovic2013equivalence}. Therefore, when $\HSIC(X,Y) = 0$, it also implies that $X$ and $Y$ are independent such that $P_{X,Y}=P(X)P(Y)$. Conversely, if $\HSIC(X,Y)$ i

==> tex/h_algorithm.tex <==
{\bf Algorithm.}
The ISM algorithm is based on Eq.~(\ref{eq:obj_2}) where the pseudo-code is provided in Algorithm~\ref{alg:ism}. In the case where the $\Phi$ is not a function of $W$, the minimizing eigenvectors immediately become the optimal $W$. However, if $\Phi$ is a function of $W$, we first initialize $\Phi_0$ using an approximation of $\Phi$ that is independent of $W$, then we iteratively update $\Phi$ using the last $W$ until $\Lambda$ converges. An approximation of a $\Phi$ independent of $W$ is based on the following proposition where the derivation is detailed in Appendix~\ref{app:approx_phi}. Several examples of this approximated $\Phi$ is provided in Table~\ref{table:init_phis} with the derivation the each kernel supplied in Appendix~\ref{app:deriv_phi_0}.

\begin{proposition}\label{prop:initial_pseudo_kernel}
    For any kernel within the ISM family that is twice differentiable at $\beta=0$, a $\Phi$ independent of $W$ can be approximated with
    \begin{align} 
    \Phi \approx -\sign(\nabla_{\beta} f(0)) \sum_{i,j} \Gamma_{i,j} A_{i,j}.
    \end{align} 
\end{proposition}



    
    
\label{convergence}
\textbf{Convergence Criteria: } Since the objective is to discover a linear subspace, the rotation of the space does not affect the solution. Therefore, instead of constraining the solution on the Stiefel Manifold, the manifold can be relaxed to a Grassmann Manifold. This implies that Algorithm~\ref{alg:ism} can reach convergence as long as the columns space spanned by $W$ are identical. To identify the overlapping span of two spaces, we can append the two matrices into $\mathcal{W} = [W_k W_{k+1}]$ and observe the rank of $\mathcal{W}$. In theory, the rank should equal to $q$, however, a hard threshold on rank often suffers from numerical inaccuracies.

One approach is to study the principal angles (`angles between flats') between the subspaces spanned by $W_k$ and $W_{k+1}$. This is based on the observation that if the maximal principal angle $\theta_{\text{max}} = 0$, then the two subspaces span the same space. The maximal principal angle between subspaces spanned by $W_k$ and $W_{k+1}$ can be found by computing $U \Sigma V^T = W_k^T W_{k+1}$ \cite{knyazev2012principal}. The cosines of the principal angles between $W_k$ and $W_{k+1}$ are the singular values of $\Sigma$, thus $\theta_{\text{max}} = \cos^{-1}(\sigma_{\text{min}})$. Computation of $\theta_{\text{max}}$ requires two matrix multiplications to form $V \Sigma^2 V^T = (W_k^T W_{k+1})^T (W_k^T W_{k+1})$ and then a round of inverse iteration to find $\sigma_{\text{min}}^2$. Although this approach confirms the convergence definitively, in practice, we avoid this extra computation by using the convergence of eigenvalues (of $\Phi$) between iterations as a surrogate. Since eigenvalues are already computed during the algorithm, no additional computations are required. Although tracking eigenvalue of $\Phi$ for convergence is vulnerable to false positive errors, in practice, it works consistently well. Therefore, we recommend to use the eigenvalues as a preliminary check before defaulting to principal angles.


 

